Latent Variable Modelling Using Variational Autoencoders: A survey

A probability distribution allows practitioners to uncover hidden structure in the data and build models to solve supervised learning problems using limited data. The focus of this report is on Variational autoencoders, a method to learn the probability distribution of large complex datasets. The report provides a theoretical understanding of variational autoencoders and consolidates the current research in the field. The report is divided into multiple chapters, the first chapter introduces the problem, describes variational autoencoders and identifies key research directions in the field. Chapters 2, 3, 4 and 5 dive into the details of each of the key research areas. Chapter 6 concludes the report and suggests directions for future work. A reader who has a basic idea of machine learning but wants to learn about general themes in machine learning research can benefit from the report. The report explains central ideas on learning probability distributions, what people did to make this tractable and goes into details around how deep learning is currently applied. The report also serves a gentle introduction for someone looking to contribute to this sub-field.

==> vgp <==
notes

GP creates a probability distribution over the function
that maps src to target

the expressiveness of the approximate posterior deoends on the complexity of the prior of the heirarchical model.

Given some data, D, we can see how the probability distribution of
the function changes.

draw epsilon
draw random non-linear mapping of the function
use function to obtain 

So is q here an inference network? What is really taking place ?

The output of GP is the mean-field parameters.
But I thought mean-field parameters were the variational parameters
learnt through VI?

In VAE:
	- the parameters of the mean-field are \mu and \sigma
	- these parameters are predicted using an amortized inference network

VGP:
	- parameters predicted using the output of a function, which is
	modelled 

\theta = set of parameters for the kernel function
D = variational data used VGP

in VAE, the parameters of the distribution q was the mean field parameters

here, the parameters are the parameters of the GP,
this GP outputs the parameters of q. So you have an aux
inference setup.

You predict \theta and D using an inference network q that
takes x as input and predicts them. 

Basically, the idea is to make the inference network
predict the parameters of a learning function and the data
for the learning function to work with. 
The learning function uses these parameters to output the
parameters of the posterior.
= What are the requirements then ?
	- here they have a learning function that generates
	random outputs


In normalizing flow:
	Sampling still takes place from the encoder network
	these samples are made complex before feeding into
	decoder

In heirarchical VI:
	The inference network predicts the parameters of each
	level

The reason VGP defined a GP and not a function is
cos you need a distribution over the latent heirarchy
a GP is a very complex distribution. Since it samples
functions, it gives this randomness required.

But wouldn't a function also give the same, since the parameters
vary? => Interesting, 

reparam trick allows us to convert \epsilon
to a complex distribution over latent variables.

The idea of VGP is to have a gaussian process
that learns this.

Things to talk about:
	-Make them understand gaussian processes enough so that they can implement
	it themselves
	-Show how GP fit into this framework. 
	-VGP has the capacity to represent complex posteriors and in the limit can represent it
	-This method is called non-parametric because its parameters are the data,
	its not restricted to mean and variance like other methods, the number of
	parameters can increase with the amount of data.
	-VGP forms infinite ensemble, cos GP is non-parametric.


	-Explain what GP is
	-what non-parametric means
	-heirarchical models, actual posterior
	-explain what VGP is doing
	-Talk about how they proved that in the limit of variational data, KL with
	the true posterior approaches zero.
	
